Phenomenological Aspects of the $E_6$SSM

The inert neutralino sector of the $E_6$SSM and the dark matter that naturally arises from this sector is studied for the first time. Limits on the parameter space from experimental and cosmological observations relating to the inert neutralino dark matter are explored and the consequences for Higgs boson phenomenology are investigated. In plausible scenarios it is found that the couplings of the lightest inert neutralinos to the SM-like Higgs boson are always rather large. This has major implications for Higgs boson collider phenomenology and leads to large spin-independent LSP-nucleon cross-sections. Because of the latter, scenarios in which $E_6$SSM inert neutralinos account for all of the observed dark matter are now severely challenged by recent dark matter direct detection experiment analyses. In plausible scenarios consistent with observations from both cosmology and LEP the lightest inert neutralino is required to have a mass around half of the Z boson mass if it contributes to cold dark matter and this means that $\tan(\beta)$ cannot be too large. A new variant of the $E_6$SSM called the $E_6Z_2^S$SSM is also presented in which the dark matter scenario is very different to the inert neutralino cold dark matter scenario and in which the presence of supersymmetric massless states in the early universe modifies the expansion rate of the universe prior to Big Bang Nucleosynthesis. The new dark matter scenario is consistent with current observations and the modified expansion rate provides a better explanation of various data than the SM prediction. The prospects for a warm dark matter scenario in the $E_6$SSM are also briefly discussed.

==> references.tex <==
\newpage
\begin{thebibliography}{99}

\bibitem{Moretti:2000}
  M.~Moretti, \textit{``A new approach to multi-jet calculations in hadron collisions,''} 
  Nucl. Phys. Proc. Suppl. {\bf 89} (2000) 190-195.

\end{thebibliography}


